Task-aware Distributed Source Coding under Dynamic Bandwidth

Efficient compression of correlated data is essential to minimize communication overload in multi-sensor networks. In such networks, each sensor independently compresses the data and transmits them to a central node due to limited communication bandwidth. A decoder at the central node decompresses and passes the data to a pre-trained machine learning-based task to generate the final output. Thus, it is important to compress the features that are relevant to the task. Additionally, the final performance depends heavily on the total available bandwidth. In practice, it is common to encounter varying availability in bandwidth, and higher bandwidth results in better performance of the task. We design a novel distributed compression framework composed of independent encoders and a joint decoder, which we call neural distributed principal component analysis (NDPCA). NDPCA flexibly compresses data from multiple sources to any available bandwidth with a single model, reducing computing and storage overhead. NDPCA achieves this by learning low-rank task representations and efficiently distributing bandwidth among sensors, thus providing a graceful trade-off between performance and bandwidth. Experiments show that NDPCA improves the success rate of multi-view robotic arm manipulation by 9% and the accuracy of object detection tasks on satellite imagery by 14% compared to an autoencoder with uniform bandwidth allocation.

==> figure_latex/CNNAutoencoder.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.75\textwidth]{figure/arch/CNN_enc.pdf}
\caption{
\small{CNN Encoder architecture.}}
\label{fig:cnn_enc}
\vspace{-1em}
\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=0.75\textwidth]{figure/arch/CNN_dec.pdf}
\caption{
\small{CNN Decoder architecture.}}
\label{fig:cnn_dec}
\vspace{-1em}
\end{figure*}

==> figure_latex/task-aware_dsc.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.60\textwidth]{figure/sys_model.pdf}
\caption{\small
    Task-aware distributed source coding.
}
\label{fig:sys_model}
\vspace{-1em}
\end{figure}

==> section/DPCA_v0.tex <==
\label{sec:DPCA}

% Since the optimal encoders and decoder of task-aware distributed source coding in \Eqref{eqn:task_loss} are difficult to obtain, we use neural networks as the autoencoder. One limitation of this approach is the fixed latent dimension for $z_i$. It poses two challenges: The first is the distribution of available bandwidth among all sources, while most of the existing works fix latent dimensions for all sources \cite{NDIC,zhang2023ldmic}. Autoencoders should allocate bandwidths based on the importance of each source to the task, but it is not trivial to measure. The second is the need to retrain autoencoders when the total available bandwidth changes. Existing works train different models for each compression level, making it prohibitive to store all the models when operating with dynamic bandwidth. To solve these problems, we propose augmenting the distributed source encoder with a distributed principal component analysis module that can redistribute the available bandwidth among the sources based on the singular values and allows us to dynamically choose the compression level based on available bandwidth. 
% By learning representations that are more linearly compressible, we achieve a graceful trade-off in performance v.s. latent dimension with only one model for multiple levels of compression. 

% (simple) Linear case (simpler) --> (2) bandwidth allocation

In this section, we consider the task-aware distributed source coding for linear tasks under the constraint of linear encoders and a decoder. 

1. We provide the optimal solution - distributed PCA. % We start with theoretically analyzing the case of a linear compressor and task and propose a novel compression method called distributed principle component analysis (DPCA). 

2. Dynamic bandwidth 

3. We then analyze the performance of DPCA and gain insights into combining DPCA with neural autoencoders later in \secref{sec:NDPCA}. 

% in addition to the difficulty of task-aware distributed source coding, autoencoders face two additional challenges when operating in bandwidth that fluctuates over time: The first is the distribution of the available bandwidth among all sources, while most existing work fixes latent dimensions for all sources \cite{NDIC,zhang2023ldmic,whang2021neuralDSC}. 
% % Ideally, autoencoders should allocate bandwidths to each source based on the importance of the task, but it is not trivial to measure while the task is a neural network. 
% The second is the need to redesign the autoencoders when the total available bandwidth changes. Existing works train different models for each compression level, making it prohibitive to store all the models when operating with dynamic bandwidth. 
% In this section, we first consider the linear setting of the problem and propose a distributed version of the principal component analysis, called DPCA. 
% We analyze the performance of DPCA and gain insights into combining DPCA with neural autoencoders later in \secref{sec:NDPCA}. 

% \textbf{Linear setting:} 
\textbf{DPCA Formulation:} 
We consider linear tasks for two sources, defined by the task matrix $\Phi\in \mathbb{R}^{\ydim\times(\xdim{1}+\xdim{2})}$, where the sources $x_1 \in \mathbb{R}^{n_1}$ and $x_2 \in \mathbb{R}^{n_2}$ are of dimension $n_1$ and $n_2$, respectively, and the task output is given as $y = \Phi x \in \mathbb{R}^{\ydim}$, where $x = [x_1^T, x_2^T]^T$. Without loss of generality, we assume the sources to be zero-mean. 

Now, given $N$ observations of %We begin by considering the case of
two sources $\X{1}\in \mathbb{R}^{\xdim{1}\times\N}$ and $\X{2}\in \mathbb{R}^{\xdim{2}\times\N}$ and their corresponding task outputs $\Y = \Phi(\X{1},\X{2}) \in \mathbb{R}^{\ydim\times\N}$, % We assume that the optimal allocation of bandwidth among the sources, $\zdim{1}$ and $\zdim{2}$ is known, and $m=\zdim{1}+\zdim{2}$. 
we aim to design the optimal linear encoding matrices (encoders) $E_1 \in \mathbb{R}^{\zdim{1}\times\xdim{1}}$, $E_2 \in \mathbb{R}^{\zdim{2}\times\xdim{2}}$, and the decoding matrix (decoder) $D \in \mathbb{R}^{(\zdim{1}+\zdim{2})\times(\xdim{1}+\xdim{2})}$ that minimizes the task loss defined as the Frobenius norm of $\Phi(X)-\Phi(\hat{X})$, where $X=[X_1^\top X_2^\top]^\top$ and $\hat{X}$ is the reconstructed $X$.  We assume that bandwidth allocation $m_1$ and $m_2$ are given for now; we discuss the optimal allocation given the total bandwidth later in this section. 
% For a task matrix $\Phi\in \mathbb{R}^{\ydim\times(\xdim{1}+\xdim{2})}$, the loss is the Frobenius norm of $\Phi(X)-\Phi(\hat{X})$, where $X=[X_1^\top X_2^\top]^\top$ and $\hat{X}$ is the reconstructed $X$. 
% 
We assume that the total bandwidth is less than the task dimension, $m_1 + m_2 < \ydim$, i.e., the encoders cannot directly calculate the task output locally and transmit it to the decoder. 

Inspired by the principle component analysis (PCA) for a single source reconstruction, which compresses one data matrix to any dimension optimally \citep{PCA}, we formulate the DPCA for a task as follows.


Letting $\Z{1}$ and $\Z{2}$ denote the encoded 


The encoders $E_1$ and $E_2$ project the data to orthonormal representations

Letting $\Z{1}\in\mathbb{R}^{\zdim{1}}$ and $\Z{2}\in\mathbb{R}^{\zdim{2}}$ denote the encoding of two sources $X_1$ and $X_2$ via $E_1$ and $E_2$, respectively, %  in \Eqref{eq:DPCA_enc}. 


%For a single source $X$, principle component analysis (PCA) compresses one data matrix to any dimension optimally \citep{PCA}. %, as shown in \Eqref{eq:PCA}. 
% Similar to PCA, 
DPCA 
aims to compress data matrices to any dimension optimally, but it reconstructs the output $\Y$ of task $\task$, as shown in \Eqref{eq:DPCA_obj}. 


The encoders $E_1$ and $E_2$ project the data to orthonormal representations $\Z{1}\in\mathbb{R}^{\zdim{1}}$ and $\Z{2}\in\mathbb{R}^{\zdim{2}}$ in \Eqref{eq:DPCA_enc}. 
We constrain the representations to be orthonormal vectors in \Eqref{eq:DPCA_orth} since we want to normalize the representations while enabling us to decouple the problem into subproblems, which is mentioned later.
% Constraint \Eqref{eq:DPCA_orth} is similar to \Eqref{eq:PCA_orth}, as they all serve as normalization constraints.
Finally, in \Eqref{eq:DPCA_dec}, the decoder $\dec$ decodes $\Z{1}$ and $\Z{2}$ to $\Xhat{1}$ and $\Xhat{2}$ and passes the reconstructed data to task $\task$. 
For simplicity, we define $\taskdec$ as the product of task $\task$ and the decoder $\dec$. Solving $\taskdec$ is identical to solving the decoder $\dec$ since we can always convert $M$ to $\dec$ by the generalized inverse of task $\task$. 
% \begin{minipage}[t]{0.5\textwidth}
% \begin{subequations}
% \begin{align}
% \operatorname*{argmin}_{\dec_{\mathrm{PCA}}, \enc{\mathrm{PCA}}} \quad & \|\X{} - \Xhat{\mathrm{PCA}}\|_2^2 \\
% \mathrm{s.t. } \quad & \Xhat{\mathrm{PCA}} = \dec_{\mathrm{PCA}} \enc{\mathrm{PCA}} \X{} \\
% \quad & \dec_{\mathrm{PCA}} \enc{\mathrm{PCA}} = \mathbf{I}_{\zdim{}}. % \in \mathbb{R}^{\zdim{}\times\zdim{}}.
% \label{eq:PCA_orth}
% \end{align}
% \label{eq:PCA}
% \end{subequations}
% \end{minipage}\begin{minipage}[t]{0.5\textwidth}
\begin{subequations}
\begin{align}
% \enc{1}^*, \enc{2}^*, \taskdec^* = \arg
\operatorname*{argmin}_{\enc{1}, \enc{2}, \taskdec} & \quad \|Y-\taskdec \Z{}\|_2^2 \label{eq:DPCA_obj} \\
\mathrm{s.t. }  
& \quad \Z{} = \begin{bmatrix}\Z{1}\\ \Z{2}\end{bmatrix} = \begin{bmatrix}\enc{1}\X{1} \\ \enc{2}\Xcom \end{bmatrix} \label{eq:DPCA_enc} \\
& \quad \Z{} \Z{}^\top  = \mathbf{I}_{\zdim{}} \label{eq:DPCA_orth}\\
& \quad \Yhat = \underbrace{\task \dec}_{\taskdec} \Z{}, ~~~\Y = \task  
\label{eq:DPCA_dec}
\begin{bmatrix}\X{1} \\ \X{2} \end{bmatrix}.
%\in \mathbb{R}^{\zdim{tot}}.
\end{align}
\label{eq:DPCA}
\end{subequations}
% \end{minipage}

\textbf{Solution:} We now formally characterize DPCA.
\label{sec:sub_DPCA}
First, a preprocessing step removes the correlation part of $\X{1}$ from $\X{2}$ by subtracting the least-square estimator $\hat{\X{2}}(\X{1})$: 
\begin{equation}
\Xcom = \X{2} - \hat{\X{2}}(\X{1}) 
= \X{2} - \X{2}\X{1}^\top(\X{1}\X{1}^\top)^{-1}\X{1}.
\label{eq:preprocess}
\end{equation}
The orthogonality principle of least-square estimators \citep[p.386]{FundamentalsSignalProcessing} ensures $\X{1}{\Xcom}^\top=\mathbf{0}_{\xdim{1}\times \xdim{2}}$.
% Then, \Eqref{eq:DPCA} shows the formulation of DPCA. 
% We now formulate the linear distributed source coding problem in \Eqref{eq:DPCA}. 
Since the decoding process minimizes the Frobenius norm is linear regression, we know that:
$$\taskdec^*= \Y\Z{}^\top(\Z{}\Z{}^\top)^{-1} = \Y\Z{}^\top.$$ 
% By \Eqref{eq:DPCA_orth} and the orthogonality principle \Eqref{eq:orth_prin}, we can rewrite the objective function in \Eqref{eq:DPCA_obj} as:
We decouple the objective in \Eqref{eq:DPCA_obj} with respect to $\enc{1},\enc{2}$ by the orthogonality principle and \Eqref{eq:DPCA_orth}:
\begin{equation}
\begin{aligned}
\operatorname*{min}_{E1, E2} \|\Y-\taskdec^* \Z{}\|_2^2 
= \|\Y\|_2^2 - \max_{\enc{1}, \enc{2}}\|\taskdec^*\|_2^2 
= \|\Y\|_2^2 - \operatorname*{max}_{\enc{1}} \|\Y_1\enc{1}\X{1}\|_2^2 - \operatorname*{max}_{\enc{2}} \|\Y_2 \enc{2}\Xcom\|_2^2,
\end{aligned}
\end{equation}
where $\Y = \begin{bmatrix}\Y_{1} ~ \Y_{2} \end{bmatrix}$.
We then have two subproblems from \Eqref{eq:DPCA}: \\
\begin{minipage}[t]{0.5\textwidth}
\begin{equation}
\begin{aligned}
\enc{1}^*=\operatorname*{argmax}_{\enc{1}} & \quad \|\Y_1\enc{1}\X{1}\|_2^2 \\
\mathrm{s.t. }  
& \quad \enc{1}\X{1}\X{1}^\top\enc{1}^\top = \mathbf{I}_{\zdim{1}},
\label{eq:DPCA_sub1}
\end{aligned}
\end{equation}
\end{minipage}\begin{minipage}[t]{0.5\textwidth}
\begin{equation}
\begin{aligned}
\enc{2}^*=\operatorname*{argmax}_{\enc{2}} & \quad \|\Y_2\enc{2}\Xcom\|_2^2 \\
\mathrm{s.t. }  
& \quad \enc{2}\Xcom{\Xcom}^\top\enc{2}^\top = \mathbf{I}_{\zdim{2}}. 
\label{eq:DPCA_sub2}
\end{aligned}
\end{equation}
\end{minipage}

The two subproblems are canonical correlation analysis \citep{CCA}, which can be solved by whitening $\enc{1}\X{1},\enc{2}\Xcom$ and singular value decomposition (see \cite{CCA} for details). 

\textbf{Dynamic bandwidth:} So far, we solved the case for fixed bandwidth $\zdim{1}$ and $\zdim{2}$. 
We now describe ways to determine the optimal bandwidth allocation given a current total bandwidth $\zdim{}$. 
DPCA solves \Eqref{eq:DPCA_sub1} and \Eqref{eq:DPCA_sub2} with $\zdim{1}=\xdim{1}$ and $\zdim{2}=\xdim{2}$ and obtain $\enc{1}^*$ and $\enc{2}^*$. DPCA then calculates all the singular values and vectors of $\taskdec_1^*\enc{1}^*\X{1}$ and $\taskdec_2^*\enc{2}^*\Xcom$. 
The sums of squares of singular values are the optimal values of \Eqref{eq:DPCA_sub1} and \Eqref{eq:DPCA_sub2}, so DPCA sorts all the singular values in descending order and chooses the first $\zdim{}$ singular values and vectors according to the available bandwidth $\zdim{}$. 
These singular vectors determine the optimal encoders $\enc{1}^*,\enc{2}^*$ and decoder $\dec^*$, which indirectly solves $\zdim{1}$ and $\zdim{2}$. Intuitively, we can conclude that the singular values indicate the importance of the task, and we prioritize the transmission of dimensions with larger singular values. For simplicity, we only consider compression of $2$ sources. However, DPCA can easily compress more sources simply by constraining all $\Z{}$s to be independent and thus decoupling the original problem \Eqref{eq:DPCA} to more subproblems.

\textbf{Performance analysis of DPCA: } Previously, we discussed how to obtain the optimal linear encoders and decoder given data matrices $\X{1}$ and $\X{2}$. We now discuss the case of DPCA compressing new data matrices $\X{1}', \X{2}'$ and the limitations of DPCA.
When DPCA is deployed and compressing new data matrices, the preprocessing step is invalid as the encoders cannot communicate with each other. 
% Hence, while DPCA is processing new data matrices $\X{1}', \X{2}'$, it has to skip the preprocessing step. 
So for DPCA to perform optimally while skipping the step, the two data matrices need to be uncorrelated, namely, $\hat{\X{2}}(\X{1})=0$, because in such case the preprocessing step is removing nothing from the data sources. 
% \begin{equation}
% \enc{2}\X{2}=\enc{2}\Xcom \Leftrightarrow \enc{2}\hat{\X{2}}(\X{1})=0. \label{eq:encgood}
% \end{equation}
% The key difference for encoding and decoding unseen data matrices $\X{1}', \X{2}'$ is during the preprocessing step in \Eqref{eq:preprocess}. 
% We previously assumed that encoder $2$ knows $\X{1}$, so it can remove the correlated part from $\X{2}$. 
% This is not the case for unseen data $\X{1}', \X{2}'$ since the encoders $\enc{1}$ and $\enc{2}$. %Hence we need to explicitly ensure that the given sources can be processed to remove the correlation for DPCA to be optimal i.e.,
% \Eqref{eq:encgood} naturally holds true when $\X{1}$ and $\X{2}$ are two uncorrelated sources
% or $\Xcom$ and $\hat{\X{2}}(\X{1})$ lie in different subspaces.  
Given that correlated sources lead to suboptimality of DPCA, we characterize the performance between PCA and DPCA under the same bandwidth in \lmaref{lemma:boundDPCA} in the simplest case without a task, which is later used in NDPCA. 
\begin{lemma}[Bound of DPCA Reconstruction]
\label{lemma:boundDPCA}
Given a zero-mean data matrix and covariance matrix, 
$$X = \begin{bmatrix}
X_1 \\
X_2
\end{bmatrix} \in \mathbb{R}^{(\xdim{1}+\xdim{2})\times N}, 
XX^\top =  \underbrace{\begin{bmatrix}
\mathrm{Cov}_{11} & \mathbf{0} \\
\mathbf{0} & \mathrm{Cov}_{22}
\end{bmatrix}}_{X_{\mathrm{diag}}}
+ \underbrace{\begin{bmatrix}
\mathbf{0} & \mathrm{Cov}_{12} \\
\mathrm{Cov}_{21} & \mathbf{0} 
\end{bmatrix}}_{\Delta X}, $$
and assume that $\Delta X$ is relatively smaller than $X_{diag}$, 
for PCA matrices $E_{\mathrm{PCA}}, D_{\mathrm{PCA}}$, and DPCA matrices $E_{\mathrm{DPCA}}, D_{\mathrm{DPCA}}$, the difference of the reconstruction losses is bounded by 
\begin{align*}
0 \leq & 
\| X - D_{\mathrm{DPCA}}\ E_{\mathrm{DPCA}}(X)\|_2^2 - \| X - D_{\mathrm{PCA}} E_{\mathrm{PCA}}(X)\|_2^2 \\
\leq  & \mathrm{Tr}(\Delta X) - 
\sum_{i=\zdim{}+1}^{\xdim{1}+\xdim{2}} \left( 2\lambda_i e_i^\top \Delta X e_i + (e_i^\top \Delta X e_i)^2 \right),
\end{align*}
where $\lambda_i , e_i$ is the $i$-th largest singular value and singular vector of $X_{\mathrm{diag}}$, $\mathrm{Tr}$ is the trace function, and $\zdim{}$ is the total bandwidth. 
\end{lemma}
The proof of \lmaref{lemma:boundDPCA} is provided in \appref{sec:app_proof}. Note that $\mathrm{Tr}(\Delta X)$ is the trace of the correlation of sources, so as $\mathrm{Tr}(\Delta X)$ gets smaller, the difference of PCA and DPCA is closer to $0$. That is, as the covariance decreases, DPCA performs more closely to PCA, which is the optimal joint compression. 

To summarize, DPCA needs the data matrices $\X{1}$ and $\X{2}$ to be orthogonal in their row spaces. If this constraint holds, DPCA can optimally choose the latent space dimensions of sources $1$ and $2$ based on their importance for the task, measured by singular values. 
Thus, DPCA finds the optimal linear encoders and decoder, given any fixed total bandwidth. 
One interesting application of DPCA is that encoders can always use the remaining unselected singular vectors to improve the quality of the transmitted data when the available bandwidth is higher.

%%%% backup 

% The two sources observing data in matrix form: $\X{1}\in \mathbb{R}^{\xdim{1}\times\N}$ and $\X{2}\in \mathbb{R}^{\xdim{2}\times\N}$, where $\xdim{i}$ is the dimension of data at source $i$, and $\N$ is the number of observations. 
% Encoders $E_1 \in \mathbb{R}^{\zdim{1}\times\xdim{1}}$, $E_2 \in \mathbb{R}^{\zdim{2}\times\xdim{2}}$, and decoder $D \in \mathbb{R}^{(\zdim{1}+\zdim{2})\times(\xdim{1}+\xdim{2})}$ are matrices that encode and decode $\X{i}$ to a lower dimension $\zdim{i}$. 
% Task $\Phi\in \mathbb{R}^{\ydim\times(\xdim{1}+\xdim{2})}$ is a matrix that takes the $\X{1}$ and $\X{2}$ to generate an output $\Y\in\mathbb{R}^{\ydim}$. 
% Without loss of generality, we assume the sources to be zero-mean. We define the task loss as the square of the Frobenius norm and the total bandwidth as $m$.


% Consider $X = \begin{bmatrix}\X{1}, \X{2}\end{bmatrix}$, where $\{X_1, X_2 \} \in \mathbb{R}^{{\xdim{1}+\xdim{2}} \times N}$ are $N$ samples of sources $1$ and $2$ respectively. 

==> section/checklist.tex <==

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}


==> section/intro.tex <==
% \begin{enumerate}
%     \item Compression of correlated data improves communication efficiency in multi-sensor networks, such as satellite networks. 
%     \item We design a data compression scheme that combines a neural autoencoder
%     with a novel principal component analysis method (refer to Fig.1 system graph). 
%     \item Our scheme adaptively chooses what to compress according to the importance of the dimension of the representations. 

%     \item Our key insights are: 
%     1. Data for correlated sources have mutual information, and we do not want to transmit redundant information from two sources through limited bandwidth. 
%     2. Different data sources have different importance, so we should allocate bandwidth to different sources based on their importance.
%     \item Our contributions are: 
%     1. Propose a novel principal component analysis method for distributed sources.
%     2. Propose a data compression scheme that
%     maximizes the task performance while adapting to changes in bandwidth by measuring the importance of each latent dimension. 
%     3. Numerically show that our method works on several domains: object detection of satellite imagery and robotic arm manipulation. 
% \end{enumerate}


% Multi-sensor networks gather a significant amount of data that needs to be sent to a central server for processing, and efficient data compression plays a pivotal role in minimizing communication overload.

Efficient data compression plays a pivotal role in multi-sensor networks to minimize communication overload. 
Due to the limited bandwidth of such networks, it is often impractical to transmit all the collected data to the central server, and in many cases, the data collected by sensors, so-called sources, are highly correlated. 
For example, satellites in low Earth orbit observe overlapping images and transmit them through limited bandwidth to a central server on Earth.
% 
% To reduce the communication burden on the network, data compression should utilize the correlation between data from different sensors. 
Most of the time, the data are only processed by downstream tasks, \textit{e.g.}, object detection models, but not the human eye. 
Hence, data compression should not transmit redundant information from correlated data and should only restore task-relevant features to minimize communication overload. 



On the one hand, ... 
% Literature refers to this communication paradigm as semantic communication  
task-aware compression \citep{qin2021semantic,xie2021deep}, which has become increasingly relevant with more large pre-trained foundation models residing on the central server and multiple sensors relaying data to the models. 
% It is important to compress each source independently at an optimal rate based on its importance to the task. 
% 
On the other hand, ... 
Further, it is important to compress each source independently to avoid additional communication overload among the sources. Information theory literature refers to this problem as distributed source coding, where each encoder compresses the data source independently, and a joint decoder decompresses the data. 
Distributed source coding is a long-standing problem in information theory, with solutions known only in some special cases \citep{slepian_wolf, DSCbook}. 

However, existing distributed compression methods perform poorly in the presence of a task model and a range of available bandwidths. 
% Our key insights are that, by optimizing task loss, neural autoencoders learn task-related representations and thus fully utilize the bandwidth. Furthermore, we can redistribute the bandwidth among the representations based on their importance to the task, which is measured by the singular values of the representation matrices.
% Because of the difficulty in modeling high-dimensional data and the inter-source correlation, 
Although, it is shown that neural networks are capable of compressing stereo images \citep{balle2016end,balle2018variational} and correlated images \citep{zhang2023ldmic}, previous works only aim to reconstruct image data but not for a downstream task. Also, they fail to compress data adaptively to different bandwidths, \textit{i.e.}, different compression levels, as neural networks always output in a fixed dimension. {\color{blue} neither of the two existing approaches are not sufficient. We formulate the task-aware src coding problem and solve it. }




%%We formulate/consider this important problem of task-aware distributed source coding as follows. %. This is what we explore... 

%-------
{\bf Problem formulation.} Consider a set of $K$ correlated sources. Let $x_i \in \mathbb{R}^{\xdim{i}}$ denote the sample from source $i$ where $i \in \{ 1,2, \dots, K \}$. Samples from each source $i$ will be compressed independently by encoder $E_i$ to a latent representation $z_i \in \mathbb{R}^{\zdim{i}}$ such that $\sum_{i=1}^{K}m_i = m$, where $m$ is the total bandwidth available. A joint decoder $D$ receives the latents  $\{z_1, z_2, \dots, z_k \}$ and reconstructs the sources $\{ \hat{x}_1, \hat{x}_2, \dots, \hat{x}_k \}$. We aim to find the optimal bandwidth allocation and the set of encoders and a decoder 
\begin{equation}
\begin{aligned}
   \operatorname*{argmin}_{ E_1, E_2, \dots, E_k, D, m_1, \dots, m_k: \sum_{m_i}=m}\mathcal{L}_{\text{task}}( \Phi(x_1, x_2, \dots, x_k) , \Phi(D(E_1(x_1),E_2(x_2), \dots, E_k(x_k) ))) \\
   \quad \text{(\textit{Task-aware} distributed source coding)},
\label{eq:task_loss}
\end{aligned}
\end{equation}
where $\mathcal{L}_{\text{task}}$ is the task loss, for example, cross-entropy loss when the task is multi-class classification.



%------ 
% This paragraph: one set of work on task-aware. another set on distributed compression. But nothing is done on task-aware + distributed compression. + There are unique challenges arising from the task-aware + dist compression (it's not just adding the two prior works together). Task-aware dist compression is a long standing open problem in information tneory - and we make progress on it. eg: bandwidth allocation is a especially challenging problem. 

% \textbf{System model:}
\iffalse
% This is not really a problem setup - but our formulation. 
We consider the case where a task model at the central node requires data from all sources and the bandwidth in the network is not consistent over time, as shown in Fig. \ref{fig:system_graph}. 
First, $K$ encoders $\enc{1}, \enc{2}, \dots, \enc{K}$ compress correlated data $\X{1}, \X{2}, \dots, \X{K}$ to representations $\Z{1}, \Z{2}, \dots, \Z{K}$ independently. A module called distributed principal component analysis (DPCA) then further compresses these representations to any dimension according to the current bandwidth and decompresses the data at the central node. 
DPCA is a module of linear matrices defined later in \secref{sec:DPCA}. 
Finally, a decoder at the central node decodes the representations $\Z{1}, \Z{2}, \dots, \Z{k}$ to $\Xhat{1}, \Xhat{2}, \dots,\Xhat{K}$ and feeds them into a task. 
We measure the quality of compression using the difference of task outputs with and without compression, which we refer to as task loss, such as the difference in detection results. Together, we call this setting minimizing task loss as \textit{task-aware} distributed source coding.
This is in contrast to existing methods that reconstruct data in pixel space.
% by minimizing mean-squared errors of images 
% However, encoders can only compress data to a priori fixed bandwidth, but not adjust to changes in bandwidth. 
% This is in contrast to traditional compression methods reconstructing the data by minimizing the mean-squared error of images in pixel space.

% Because of the difficulty in modeling high-dimensional data and the inter-source correlation, neural-network-based distributed encoders have received increasing attention in recent times. Previous works study the problem of stereo image compression using deep neural networks in \citep{balle2016end,balle2018variational}. More recently, the compression of correlated images by explicitly capturing the interview correlations using the attention mechanism was studied in \citep{zhang2023ldmic}. Meanwhile, distributed source compression with side information was explored in \citep{whang2021neuralDSC,NDIC}. 

% Our proposed method compresses and decompresses the representations $\Z{1}...\Z{k}$ to any available bandwidth. 

% It is difficult to design independent encoders that collaborate on data compression without communicating with each other while transmitting task-relevant features.



% Also, previous works design neural distributed autoencoders with side information in \citep{whang2021neuralDSC,NDIC}. 


% Despite their success, these methods focus on image reconstruction for the best visual quality and do not involve any further task. But for most multi-sensor applications, the end user is rarely a human, and the data is often directly passed to a pretrained task model for inference. The effectiveness of task-aware or semantic compression has been well studied in a single source setting \citep{lossyCompressionLosslessPrediction,nakanoya2023co}. Extending the same to a multi-source setting is non-trivial since the optimal distribution of the total available bandwidth among sources still remains open \citep{modulotwo}. 
% Moreover,limitation of neural autoencoders is that they require a fixed latent dimension during the training process. As a result, it becomes necessary to train separate models for each compression level, which adds to the computational and storage requirements. 

% There are three challenges with task-aware distributed source coding. 
% The first is to determine the important features of the task at each source and only transmit these features. 
% The importance of features hidden in the data is implicit and difficult to define. Only by measuring the importance of features, we can utilize the limited bandwidth to optimally transmit task-relevant features.
% The second is to distribute the available bandwidth to sources based on the importance of the task. The optimal allocation of bandwidth among sources remains an open problem, even in the simplest setting where the task is the two-module sum of two binary sources \cite{modulotwo}. 
% The third is to use the correlation among sources to improve the overall efficiency of the bandwidth. This is non-trivial since each source has only local information and cannot communicate with other sources to estimate the correlation. Therefore, it is difficult to prevent the transmission of redundant information. 

\fi 


As a solution: We design neural distributed principal component analysis (NDPCA)–a compression framework that transmits task-relevant features in any available bandwidth.  

\begin{itemize}
    \item Analytical solution for the linear case (DPCA) 
    \item Combine NN and DPCA (refer to figure 1) 
    \item Empirical results (summary) 
\end{itemize}

NDPCA learns latent representations at multiple compression levels simultaneously without the need for retraining.
% As shown in \figref{fig:system_graph}, 
It uses a neural autoencoder to learn uncorrelated task-relevant features and thus prevent transmitting redundant information. DPCA then compresses the representations and allocates the current bandwidth among sources based on their importance of the task. 
Unlike other compressors that optimize for reconstruction error, NDPCA directly optimizes task loss and generates low-rank latent representations that are more compressible in limited bandwidths.
% with a novel random projection procedure during training. 
NDPCA only has one model for any compression level, while providing a graceful trade-off between performance and bandwidth. 

\input{figure_latex/system_model}

Our contributions are three-fold. First, we formulate a distributed variant of the task-aware source coding problem, that optimizes the bandwidth utilization for a given task instead of recovering the sources. Second, we propose a novel task-aware distributed source coding framework, NDPCA, that learns a single model for different levels of compression. Third, we provide a theoretical justification for the framework by analyzing the case of linear encoder and task. 

We validate NDPCA in several domains, such as CIFAR-10 image denoising, multi-view robotic arm manipulation, and object detection of satellite imagery. 
Experimental results show a $1.2$dB improvement in PSNR, a $9\%$ improvement success rate, and a $14\%$ improvement in accuracy in all three domains compared to an autoencoder with uniform bandwidth allocation.

% We show that NDPCA can operate efficiently at different levels of compression with a single model, vastly reducing the compute and storage overhead. 
% The proposed scheme achieves an improvement in the success rate of up to $29\%$ for a robotic arm locate and lift task and an improvement in mAP50 performance of up to $27\%$ for an object detection task on satellite imagery. 




% First, We formulate a new setting of task-ware distributed source coding, instead of existing methods that focus on reconstructing data.
% Second, we propose a novel distributed source coding framework, NDPCA, that compresses correlated data for a pretrained task to any bandwidth with a single autoencoder and no retraining. 
% Third, we provide a theoretical analysis of DPCA in linear cases and characterize the advantages of task-aware compression. 
% % Experimental results 
% To support the contributions, we validate NDPCA on multiple domains, such as CIFAR-10 data denoising \cite{CIFAR10}, multi-view robotic arm manipulation \citep{FERM}, and object detection of satellite imagery \citep{airbusKaggle}. 
% We show that NDPCA can operate efficiently at different levels of compression with a single model, vastly reducing the compute and storage overhead. 
% The proposed scheme achieves an improvement in the success rate of up to $29\%$ for a robotic arm locate and lift task and an improvement in mAP50 performance of up to $27\%$ for an object detection task on satellite imagery. 

% Addressing both aspects of this problem, we propose a compression scheme that learns the task-relevant representations of the data in a distributed set-up and also chooses the rate of compression based on the importance of each source for a given task.




% Hence we introduce a distributed variant of principal component analysis (PCA) into the neural auto-encoder network to enable adaptive selection of the latent dimension. 
% Finally, we measure the quality of compression using the degradation of the task performance with and without compression, which we refer to as task loss, such as the difference in detection results. Together, we call this setting minimizing task loss as \textit{task-aware} distributed source coding. This is in contrast to traditional compression methods reconstructing the data by minimizing the mean-squared error of images in pixel space. 



% each source independently to avoid additional communication overload among the sources while also choosing the optimal rate of compression for each


% Information theory literature refers to this problem as distributed source coding, where each encoder compresses the data source independently, and a joint decoder decompresses the data while leveraging the correlation between the sources \citep{slepian_wolf, DSCbook}. 



% efficient data compression plays a pivotal role in minimizing communication overload. In many scenarios, the data collected is often correlated because of the proximity or other factors and efficiently utilizing 

% Efficient compression of correlated data is essential to minimize communication overload in multi-sensor networks because many applications collect large amounts of correlated data. 

% Transmitting entire collected data  to a central node, so-called cloud, is often prohibitive due to limited bandwidth. Hence, it is crucial to efficiently compress the data to representations relevant to the downstream task while avoiding encoding redundant information. Literature refers to this communication paradigm as semantic communication \citep{qin2021semantic,xie2021deep}, which is increasingly relevant with more large pretrained foundation models residing in the cloud and multiple sensors, so called sources, relaying data to the pretrained models. It is important to compress each source independently to avoid additional communication overload among the sources. Information theory literature refers to this problem as distributed source coding, where each encoder compresses the data source independently, and a joint decoder decompresses the data while leveraging the correlation between the sources \citep{slepian_wolf, DSCbook}.

% We propose a distributed compression framework that focuses on learning independent encoders and a joint decoder to learn task-aware representations that are efficient in any bandwidth. 
% \textbf{System model:}
% We consider the case where a task model $\task$ at the central node requires data from multiple sources as input, and the bandwidth in the network is limited and inconsistent over time, as shown in \figref{fig:system_graph}. Encoders $\enc{1}, \enc{2}, \dots, \enc{k}$, compress the corresponding correlated sources $\X{1}, \X{2}, \dots, \X{k}$ to send to a common decoder $\dec{}$ at the central node. For example, consider a low earth orbit (LEO) satellite constellation transmitting aerial images to a base station. It is likely for the views of different satellites to be overlapping, introducing correlation among the views.



% Because of the difficulty in modeling high-dimensional images, we choose neural networks to be our choice of encoders and decoder. Despite the advantages,




% \textit{e.g.},



% \textit{e.g.}, a low earth orbit (LEO) satellite constellation transmitting  



% neural networks on satellites, compress correlated data $\X{1}, \X{2}, \dots, \X{k}$, \textit{e.g.}, overlapping images of the Earth, to representations $\Z{1}, \Z{2}, \dots, \Z{k}$ independently and send them to a decoder $\dec{}$ at a central node, \textit{e.g.,} the Earth. 
% Compression is necessary due to the limited bandwidth. 
% However, encoders can only compress data to a priori fixed bandwidth, but not adjust to changes in bandwidth. Our proposed method can compress and decompresses the representations $\Z{1}, \Z{2}, \dots, \Z{k}$ to any available bandwidth by further compressing the representations with linear matrices. 
% Then, the decoder $\dec$ decodes the representations $\Z{1}, \Z{2}, \dots, \Z{k}$ to $\Xhat{1}, \Xhat{2}, \dots, \Xhat{k}$ and feeds them into a task $\task$, \textit{e.g.,} an object detection model. 


% Efficient compression of correlated data is crucial for minimizing the communication overload in multi-sensor networks, such as satellite networks. 
% In the network, sensors observe correlated data, \textit{e.g.}, images taken from satellites, compress the data and transmit them to a central node, \textit{e.g.}, a mission control center on Earth. 
% Data compression is critical because the communication bandwidth of the network is limited, and the real-time sensory data is huge due to the number of sensors and the size of the data itself.
% Information theory literature refers to this setting as distributed source coding, where an encoder compresses only $1$ data source, and a decoder decompresses the outputs of all encoders jointly. 

% \textbf{Challenges:}
% There are three challenges with task-aware distributed source coding. 
% The first is to determine the important features of the task at each source and only transmit these features. 
% The importance of features hidden in the data is implicit and difficult to define. Only by measuring the importance of features, we can utilize the limited bandwidth to optimally transmit task-relevant features.
% The second is to distribute the available bandwidth to sources based on the importance of the task. The optimal allocation of bandwidth among sources remains an open problem, even in the simplest setting where the task is the two-module sum of two binary sources \cite{modulotwo}. 
% The third is to use the correlation among sources to improve the overall efficiency of the bandwidth. This is non-trivial since each source has only local information and cannot communicate with other sources to estimate the correlation. Therefore, it is difficult to prevent the transmission of redundant information. 

% \textbf{Proposed method:}
% To address these challenges, we propose neural distributed principal component analysis (NDPCA) to generate compressible task representations and efficiently distribute any available bandwidth among sources. 
% % generate efficient representations of data sources and dynamically project the representations to any communication bandwidth. 
% NDPCA combines a neural autoencoder with a novel principal component analysis method, distributed principal component analysis (DPCA). 
% % The neural autoencoder of NDPCA generates uncorrelated representations of data sources, so the limited network bandwidth is not used to transmit redundant information. 
% Unlike existing autoencoders that only compress data to an a priori fixed bandwidth, DPCA compresses representations to any dimension and redistributes available bandwidth based on the importance of the representations for the task. NDPCA then decompresses the representations back to the original data space. 
% % Finally, a task model inputs the decompressed data to compute the output. 
% Note that NDPCA only has one autoencoder model and needs no retraining for different compression levels.



% \textbf{Key observation and insights:}
% Our key observations are that existing distributed compression methods optimized for data reconstruction perform poorly in the presence of a task model and only compress data to a priori fixed bandwidth. 
% Our key insights are that, by optimizing task loss, neural autoencoders learn task-related representations and thus fully utilize the bandwidth. Furthermore, we can redistribute the bandwidth among the representations based on their importance to the task, which is measured by the singular values of the representation matrices.
% by introducing a linear compression module, DPCA, into the framework, we can redistribute the bandwidth among the representations based on their importance to the task, further improving efficiency. 


% The experimental results indicate savings of up to $62.5\%$ in bandwidth, with only slight degradation in performance. 

    % (1) distributed & task aware setup itself. % We provide a constructive algorithm & for linear case, we provide a theoretical analysis
    % 
    % (2) Task fixed. Pre-trained model for the task which takes Xhat and Yhat as inputs: (Robust training)
    % (Q) Why pre-training?? Big models already.  
    % (State-of-the-art) encode each X, Y, Z, separately -- Why is that not good? A. Task-relevant. B. (not utilizing correlation) C. How much -bandwidth allocation? 
    % (So what do we propose to do?): 
    % (So what do we show?): 
    % Each figure ; clear message. 
    % don't wanna train too many models () why? Flexible compression length (eg video streaming) Dynamic bandwidth/resource constraints. 
    % (3) Allocation across sources: Task-dependency  
    % (4) Correlation (?) 


% show that the proposed scheme achieves $62.5\%$ times bandwidth savings in a simulated robotic arm task and $66.7\%$ times savings in an object detection task for satellite imagery.


% 1. We proposed a loss function for neural networks to generate more compressible representation spaces. 
% 2. We show that our data compression scheme, NDPCA, can transmit data in any network bandwidth without retraining neural networks or redesigning network architecture. 
% 3. We examine our method on the a robotic manipulation task \citep{FERM} and a satellite object detection task \citep{airbusKaggle}. Experimental results show that the proposed scheme achieves $62.5\%$ times bandwidth savings in a simulated robotic arm task and $66.7\%$ times savings in an object detection task for satellite imagery.
% Our key insights are that neural networks are powerful enough to generate uncorrelated representations, and we should transmit data based on their importance to the task as we only have limited network bandwidth. Hence, we use NDPCA to generate uncorrelated representations and use DPCA to measure the importance of each dimension of representations. 


% 1. We design a data compression scheme that combines a neural autoencoder with a novel principal component analysis method, distributed principal component analysis (DPCA). The autoencoder generates independent representations, and DPCA compresses these representations near-optimally.  
% 2. We show that our data compression scheme can fit in any network bandwidth with only one model without retraining neural networks,  while sacrificing minimal task performance. 
% 3. We prove that DPCA is optimal given uncorrelated representations and provide performance bounds for our compression scheme compared to the optimal compression. 





% There are two factors that contribute to the difficulty of task-aware distributed source coding: 1. correlation of data sources. 2. importance of each source to the task. First, all data sources observe correlated data but each source only has local information, that is, each source has no knowledge of the data observed at other sources. Hence, it is difficult to prevent each source from transmitting mutual information, \textit{i.e.}, data shared among multiple sources. The second factor is that the data from each source have different levels of importance to the task. The task may utilize all information from a certain source but not anything from another source, and all sources share the same communication bandwidth to the central server. Therefore, the task determines the optimal allocation of bandwidth among all sources. The optimal allocation of bandwidth among sources is still an open problem even in the simplest setting in which the task is to calculate the sum of two binary sources \cite{modulotwo}. 

% Our data compression, which we called  neural distributed principal component analysis (NDPCA), generates representations of data sources and dynamically projects the representations to any communication bandwidth. 
% NDPCA combines a neural autoencoder with a novel principal component analysis method, as shown in Fig. \ref{fig:system_graph}.
% and categorizes representations into shared and private representations. The share representations preserve mutual information from all sources, and the private representations preserve conditional entropy, \textit{i.e.}, local information.

%% Correlation + Task - is great. 
%% [Lossless compression] For example, correlated binary sources: H(X+Y) is all you need to reconstruct X+Y. - no, this does not support the first claim. 
% This is as if X and Y are sitting together. 

%% 

% Constructive algorithms are not quite there.  

%% Cf. Lossy compression: a lot is unknown. 

% Our proposed DistTaskAE is the first constructive algorithm. 


% Even though X and Y are independent, task-awareness is useful: better compression is possible. 

%% Gaussian sources: mu-sum rate? 
%% 



% For tasks beyond sum (of binary sources), the optimal rates are unknown; constructive algorithms are unknown, either. 
%  Even for Gaussian correlated sources, the rate-distortion region for sum rate computation is unknown. 
% The state-of-the-art achievability result is by Burger-Tung. 
% 

%% Wireless transmission: Noisy transmission 

% Contributions 
% \begin{itemize}
%     \item Setup. Task-aware distributed compression - new setting. 
%     \item Algorithm: AE based compressor + VIC-reg \\ 
%     `` Private + shared (task-aware correlation)"  \\ 

% Flexible latent dimension (no retraining) using (D)PCA: improve the efficiency of compression by optimizing for correlation [private+shared]\\ 

% \item Theoretical 1:  Task-aware dist. compression (linear tasks): DPCA is optimal. 

% \item Theoretical 2: Information-theoretic 

% \item Theoretical 3: Robustness: Robust task + (i) noise from data compression and (ii) noise from wireless channel \\

% Taking the robust task vs non-robust task \\

% - Evaluating the robustness of learned dist. compression: task-aware vs. reconstruction \\ 

% \item Experimental results 

% \end{itemize}



